RELICS: Strong Lensing Analysis of MACS J0417.5-1154 and Predictions for Observing the Magnified High-Redshift Universe with JWST

Strong gravitational lensing by clusters of galaxies probes the mass distribution at the core of each cluster and magnifies the universe behind it. MACS J0417.5-1154 at z=0.443 is one of the most massive clusters known based on weak lensing, X-ray, and Sunyaev-Zel'dovich analyses. Here we compute a strong lens model of MACS J0417 based on Hubble Space Telescope imaging observations collected, in part, by the Reionization Lensing Cluster Survey (RELICS), and recently reported spectroscopic redshifts from the MUSE instrument on the Very Large Telescope (VLT). We measure an Einstein radius of ThetaE=36'' at z = 9 and a mass projected within 200 kpc of M(200 kpc) = 1.78+0.01-0.03x10**14Msol. Using this model, we measure a ratio between the mass attributed to cluster-member galaxy halos and the main cluster halo of order 1:100. We assess the probability to detect magnified high-redshift galaxies in the field of this cluster, both for comparison with RELICS HST results and as a prediction for the James Webb Space Telescope (JWST) Guaranteed Time Observations upcoming for this cluster. Our lensing analysis indicates that this cluster has similar lensing strength to other clusters in the RELICS program. Our lensing analysis predicts a detection of at least a few z~6-8 galaxies behind this cluster, at odds with a recent analysis that yielded no such candidates in this field. Reliable strong lensing models are crucial for accurately predicting the intrinsic properties of lensed galaxies. As part of the RELICS program, our strong lensing model produced with the Lenstool parametric method is publicly available through the Mikulski Archive for Space Telescopes (MAST).

==> img_mul.tex <==
%

\begin{figure*}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/1mp1.png}
\includegraphics[width=0.4\textwidth]{img/mul/1mp2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/1mp3.png}
\includegraphics[width=0.4\textwidth]{img/mul/1mp4.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/2ap1.png}
\includegraphics[width=0.4\textwidth]{img/mul/2ap2.png}
}
\caption{ Each panel presents the multiply-imaged systems or candidate from our analysis. HST RGB images.}
\end{figure*}

\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/2ap3.png}
\includegraphics[width=0.4\textwidth]{img/mul/3p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/3p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/3p3.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/4p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/4p2.png}
}\end{figure*}

\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/4p3.png}
\includegraphics[width=0.4\textwidth]{img/mul/5p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/5p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/5p3.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/6p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/6p2.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/6p3.png}
\includegraphics[width=0.4\textwidth]{img/mul/7p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/7p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/8p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/8p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/9p1.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/9p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/10p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/10p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/10p3.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/11p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/11p1.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/12p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/12p2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/12p3.png}
\includegraphics[width=0.4\textwidth]{img/mul/13p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/13p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/13p3.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/14p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/14p2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/15p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/15p2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/15p3.png}
\includegraphics[width=0.4\textwidth]{img/mul/16p1.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/16p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/16p3.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/17p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/17p2.png}
}
%\centerline{

%}
\end{figure*}
\begin{figure*}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c18p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/c18p2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c19p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/c19p2.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c20p1.png}
\includegraphics[width=0.4\textwidth]{img/mul/c21p1.png}
}
\caption{candidate}
\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c21p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/c22p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c22p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/c23p1.png}
}
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c23p2.png}
\includegraphics[width=0.4\textwidth]{img/mul/c24p1.png}
}\end{figure*}
\begin{figure*}\ContinuedFloat
\centerline{
\includegraphics[width=0.4\textwidth]{img/mul/c24p2.png}
}
\end{figure*}


